DeepCloak: Adversarial Crafting As a Defensive Measure to Cloak Processes

Over the past decade, side-channels have proven to be significant and practical threats to modern computing systems. Recent attacks have all exploited the underlying shared hardware. While practical, mounting such a complicated attack is still akin to listening on a private conversation in a crowded train station. The attacker has to either perform significant manual labor or use AI systems to automate the process. The recent academic literature points to the latter option. With the abundance of cheap computing power and the improvements made in AI, it is quite advantageous to automate such tasks. By using AI systems however, malicious parties also inherit their weaknesses. One such weakness is undoubtedly the vulnerability to adversarial samples. In contrast to the previous literature, for the first time, we propose the use of adversarial learning as a defensive tool to obfuscate and mask private information. We demonstrate the viability of this approach by first training CNNs and other machine learning classifiers on leakage trace of different processes. After training highly accurate models (99+% accuracy), we investigate their resolve against adversarial learning methods. By applying minimal perturbations to input traces, the adversarial traffic by the defender can run as an attachment to the original process and cloak it against a malicious classifier. Finally, we investigate whether an attacker can protect her classifier model by employing adversarial defense methods, namely adversarial re-training and defensive distillation. Our results show that even in the presence of an intelligent adversary that employs such techniques, all 10 of the tested adversarial learning methods still manage to successfully craft adversarial perturbations and the proposed cloaking methodology succeeds.

==> overview.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Overview of Android}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Android continues to dominate the smartphone market with an 82.8\% share as of 2015 Q2~\cite{android_market_share}. Unsurprisingly, mobile malware development almost exclusively focuses on the Android platform, with a combined total of 355 new families and variants of malware found in 2014~\cite{fsecure_h1,fsecure_h2}. The most common families of Android malware include SmsSend, SmsSpy, and FakeInst, trojans that sends SMS messages to premium-rate numbers, and Eropl, a trojan that exfiltrates personal data.

The Android platform is composed of three fundamental building blocks: the device hardware, the Android OS, and the Android application runtime, each sitting atop the previous. While Android is processor-agnostic, it can take advantage of hardware-specific security features such as ARM v6 eXecute-Never when present. The Android OS, built on top of the Linux kernel, inherits its robust security capabilities. This includes the user-based permission model, process isolation, and an extensible mechanism for secure interprocess communication (IPC). The Linux kernel is responsible for executing core system services like process management, network management, and memory access. The device resources, such as GPS, telephony, and the camera, are all accessed through the OS~\cite{android_security}.
%
In addition to inheriting Linux's security features, Android also inherits Linux's copy-on-write (COW) capability in its process creation mechanism. The root process, called Zygote, pre-loads core resources that all Android processes will use. COW allows Android to spawn new processes without memory duplication; since these core resources are read-only, the libraries common to all processes will only be stored in one location. This significantly reduces an application's memory footprint.

Prior to Android 5.0, the Dalvik VM and Android's core native services and libraries comprised the Android application runtime. Dalvik was replaced by Android Runtime (ART) in Android 5.0. Android applications are most commonly written in Java, which is compiled to bytecode for the Java Virtual Machine (JVM), and then translated to Dalvik bytecode. Native applications and libraries, such as those managing audio, SSL, and graphics,  are written in C and C++ to interface with the OS more closely and achieve better performance. The Android application runtime is contained within the Application Sandbox, a security environment which prevents applications from interfering with each other and system services. The Application Sandbox is implemented at the kernel level, and thus encapsulates and protects all components sitting above the kernel.


The Application Sandbox is realized through two fundamental Linux features: user-based access-control and memory isolation. The former implements standard file access rights by allowing each user to control who is allowed to read, write, and execute their files. The Application Sandbox leverages this by assigning each application it's own unique user identifier (UID), thus preventing one application from accessing the files of another. Android requires each application to be signed by its developer before being uploaded to the Play Store. Applications that are signed with the same key are assigned the same Linux UID within Android, bypassing the isolation model provided by the Application Sandbox. This allows applications to share data and application components. Since there is no central Certificate Authority (CA) for developer private keys, it is the developers responsibility to keep her private key secure. If she fails, adversaries can abuse the shared UIDs to access sensitive information.

Further, system components are run as root, so no user-level application can access or modify them. In Linux, each process is given its own virtual address space as a form of memory isolation. Android takes advantage of this by running each application as a separate process so no application can interfere with the memory space of another. Theoretically, since all applications are sandboxed at the OS level, memory corruption errors cannot compromise the device; they will only allow code execution with the permissions of the vulnerable application. To break out of the Application sandbox, adversaries must compromise the kernel.

In addition to the Application Sandbox, Android provides security through user-granted per app permission system. Examples of permissions include access to a user's personal information, the device's camera, and telephony and SMS capabilities. Android 6.0 introduced runtime permissions, allowing users to toggle individual permissions after installation at their discretion. %\cite{android_privilege_escalation} demonstrated a weakness in Android's permission system that allows non-privileged applications to escalate their privileges by invoking higher-privileged applications with unprotected interfaces. Android provides a way to mitigate this, but requires developers to include reference monitor hooks in higher-privileged code. This delegation of responsibility to the developer results in vulnerable applications due to inexperience or ignorance. %Finally, due to shared UIDs, applications can escalate their own privileges through IPC with higher-privileged applications signed with the same private key. For example, if a developer has two applications, one with SMS permissions and another with Internet permissions, the end-user's SMS data could be leaked to the Internet.



\subsection{Android Permission System}

Android employs permission management system to give apps access to various specific operations, sensors and data. While some of these permissions require user consent, others do not. Before Android 6.0 (API 23), the permission consent was set to be given at install time. Granting permissions at the install time meant that apps listed all the permissions that they *might* require during their operations and the users raced to the install button without checking them. After Android 6.0, permission requests are presented when the app needs that specific permission for the first time. %In cases where user declines to give the requested permission, some applications keep working while others crash outright. 

However, not all permissions require user consent. Depending on the importance of information or service that an app needs to access, permission might be automatically granted without prompting user. In the following, we explain these different types of permissions and how they are handled by the Android.


\subsubsection{Normal Permissions}
Normal permissions cover areas where the app needs to access data or resources outside the app' s sandbox, but where there is very little risk to the user's privacy or the operation of other apps. For example, permission to set the time zone is a normal permission. If an app declares that it needs a normal permission, the system automatically grants the permission to the app. Full list of Normal Permissions (As of API 23+) are listed in Appendix~\ref{app:normal_permissions}


%The default value. A lower-risk permission that gives requesting applications access to isolated application-level features, with minimal risk to other applications, the system, or the user. The system automatically grants this type of permission to a requesting application at installation, without asking for the user's explicit approval (though the user always has the option to review these permissions before installing).


\subsubsection{Dangerous Permissions}
Dangerous permissions cover areas where the app wants data or resources that involve the user's private information, or could potentially affect the user' s stored data or the operation of other apps. For example, the ability to read the user's contacts is a dangerous permission. If an app declares that it needs a dangerous permission, the user has to explicitly grant the permission to the app.\msi{shorten this}. 

The following permission groups are considered dangerous permission by the Android system and require explicit user consent; Calendar, Camera, Contacts, Location, Microphone, Phone, Sensors, SMS and Storage.

%	A higher-risk permission that would give a requesting application access to private user data or control over the device that can negatively impact the user. Because this type of permission introduces potential risk, the system may not automatically grant it to the requesting application. For example, any dangerous permissions requested by an application may be displayed to the user and require confirmation before proceeding, or some other approach may be taken to avoid the user automatically allowing the use of such facilities.

\subsubsection{Signature Level Permissions}
Closed by Vendors most of the time. Vendor dependent. Permission dependent.

Unless you put the necessary permission's request into both Manifest and the App Code, it does not prompt the user.

Real\_Get\_Tasks requires signature/system level permission. For more information about signature level permissions, read up. These permissions cannot be requested in the code (in normal mode). Requires  API 22 minimum.

%A permission that the system grants only if the requesting application is signed with the same certificate as the application that declared the permission. If the certificates match, the system automatically grants the permission without notifying the user or asking for the user's explicit approval.


\subsubsection{Signature Level Permissions}
A permission that the system grants only to applications that are in the Android system image or that are signed with the same certificate as the application that declared the permission. Please avoid using this option, as the signature protection level should be sufficient for most needs and works regardless of exactly where applications are installed. The "signatureOrSystem" permission is used for certain special situations where multiple vendors have applications built into a system image and need to share specific features explicitly because they are being built together.



